UniIR: Training and Benchmarking Universal Multimodal Information Retrievers

Existing information retrieval (IR) models often assume a homogeneous format, limiting their applicability to diverse user needs, such as searching for images with text descriptions, searching for a news article with a headline image, or finding a similar photo with a query image. To approach such different information-seeking demands, we introduce UniIR, a unified instruction-guided multimodal retriever capable of handling eight distinct retrieval tasks across modalities. UniIR, a single retrieval system jointly trained on ten diverse multimodal-IR datasets, interprets user instructions to execute various retrieval tasks, demonstrating robust performance across existing datasets and zero-shot generalization to new tasks. Our experiments highlight that multi-task training and instruction tuning are keys to UniIR's generalization ability. Additionally, we construct the M-BEIR, a multimodal retrieval benchmark with comprehensive results, to standardize the evaluation of universal multimodal information retrieval.

==> sec/model.tex <==



==> tables_and_figures/table_cross_domain.tex <==
\definecolor{positive}{HTML}{008000} % You can use a custom color for positive changes
\definecolor{negative}{HTML}{FF0000}

\begin{table}[ht!]
    \centering
    \scriptsize
    \begin{tabular}{llp{0.2cm}p{0.2cm}p{0.6cm}p{0.2cm}p{0.6cm}p{0.2cm}}
    \toprule
     &   & \multicolumn{2}{c}{\textbf{Zero-Shot}} & 
    \multicolumn{2}{c}{\textbf{UniIR} (CLIP$_{\text{SF}}$)} & \multicolumn{2}{c}{\textbf{UniIR} (BLIP$_{\text{FF}}$)}\\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
        \textbf{Task}        & \textbf{Dataset}           &  CLIP & BLIP  &  \ding{55} inst & \checkmark inst  & \ding{55} inst & \checkmark inst \\
        \midrule
         $q_i \to r_t$ & VNews & 51.6 & 18.7\\
         $q_t \to r_i$ & VNews & 49.7 & 18.4\\
         $q_t \to $ ($r_t, r_i$) & EDIS & 52.6 & 32.7\\
         \bottomrule
    \end{tabular}
    \caption{\textbf{Held-out domain generalization} experiments: we train one UniLR model on 4 held-in domains from M-BEIR and perform zero-shot evaluation on 1 held-out domain (i.e., News). Retrieval is conducted from individual task candidate pool.}
    \label{tab:cross_dataset}
\end{table}

==> tables_and_figures/table_cross_task.tex <==
\definecolor{positive}{HTML}{008000} % You can use a custom color for positive changes
\definecolor{negative}{HTML}{FF0000}

\begin{table}[ht!]
    \centering
    \scriptsize
    \begin{tabular}{llp{0.2cm}p{0.2cm}p{0.6cm}p{0.2cm}p{0.6cm}p{0.2cm}}
    \toprule
     &   & \multicolumn{2}{c}{\textbf{Zero-Shot}} & 
    \multicolumn{2}{c}{\textbf{UniIR} (CLIP$_{\text{SF}}$)} & \multicolumn{2}{c}{\textbf{UniIR} (BLIP$_{\text{FF}}$)}\\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
        \textbf{Task}        & \textbf{Dataset}           &  CLIP & BLIP  &  \ding{55} inst & \checkmark inst  & \ding{55} inst & \checkmark inst \\
        \midrule
         $q_i \to$ 
         & EDIS              & 52.6 & 32.7\\
         ($r_t, r_i$)
         & WebQA                &  53.8 & 28.4 \\         
         \midrule
         ($q_i, q_t$) 
         
         & OVEN       &                 30.7 & 18.0 \\
         
         
         
         $\to$ $r_t$ & InfoSeek      &      28.8 & 11.4\\
         \bottomrule
    \end{tabular}
    \caption{\textbf{Held-out task generalization} experiments: we train one UniLR model on 6 held-in tasks from M-BEIR and perform zero-shot evaluation on 2 held-out tasks. Retrieval is conducted from individual task candidate pool.}
    \label{tab:cross_dataset}
\end{table}
